A Symphony Conducted by Brunet

We introduce BruNet, a general P2P software framework which we use to produce the first implementation of Symphony, a 1-D Kleinberg small-world architecture. Our framework is designed to easily implement and measure different P2P protocols over different transport layers such as TCP or UDP. This paper discusses our implementation of the Symphony network, which allows each node to keep $k \le \log N$ shortcut connections and to route to any other node with a short average delay of $O(\frac{1}{k}\log^2 N)$. %This provides a continuous trade-off between node degree and routing latency. We present experimental results taken from several PlanetLab deployments of size up to 1060 nodes. These succes sful deployments represent some of the largest PlanetLab deployments of P2P overlays found in the literature, and show our implementation's robustness to massive node dynamics in a WAN environment.

==> Makefile <==
BASENAME = brunet-paper0

FIGS=Rings2.eps Shortcuts_linear.eps TimeSeries.eps Unstructured.eps churn_stats.eps \
graph_fig.eps ring1_2_fixed.eps ring2_2_fixed.eps ring_merge_1.eps ring_merge_2.eps \
ring_merge_3.eps ring_merge_4.eps ringfinal2_fixed.eps structured.eps \

BIBTEX = /usr/bin/bibtex
DVIPS  = /usr/bin/dvips
LATEX  = /usr/bin/latex
RM     = /bin/rm
CP     = /bin/cp

FIG1	 = example
NEATO		 = /usr/bin/neato

all : $(BASENAME).ps $(BASENAME).pdf

pdffigs : $(FIGS) 
	ls *.eps | xargs -n 1 epstopdf

$(BASENAME).ps : $(BASENAME).dvi
	$(DVIPS) -o $(BASENAME).ps $(BASENAME).dvi

$(BASENAME).dvi : $(FIG1).ps $(BASENAME).tex $(BASENAME).bbl
	$(LATEX) $(BASENAME); $(LATEX) $(BASENAME)

$(FIG1).ps : $(FIG1).dot
	$(NEATO) -Tps $(FIG1).dot -o $(FIG1).ps

$(BASENAME).bbl : $(BASENAME).aux
	-$(BIBTEX) $(BASENAME)

$(BASENAME).aux : $(BASENAME).tex
	$(LATEX) $(BASENAME)

#$(BASENAME).pdf : $(BASENAME).ps
#	ps2pdf -dPDFSETTINGS=/prepress $(BASENAME).ps $(BASENAME).pdf

$(BASENAME).pdf : $(BASENAME).tex pdffigs
	pdflatex $(BASENAME).tex
	pdflatex $(BASENAME).tex

.PHONY : clean
clean :
	$(RM) -f $(BASENAME).aux $(BASENAME).bbl $(BASENAME).blg \
	$(BASENAME).dvi $(BASENAME).lof $(BASENAME).log $(BASENAME).ps \
	$(BASENAME).toc *.ps *.pdf *.dvi

